Understanding the Role of Images on Stack Overflow

Images are increasingly being shared by software developers in diverse channels including question-and-answer forums like Stack Overflow. Although prior work has pointed out that these images are meaningful and provide complementary information compared to their associated text, how images are used to support questions is empirically unknown. To address this knowledge gap, in this paper we specifically conduct an empirical study to investigate (I) the characteristics of images, (II) the extent to which images are used in different question types, and (III) the role of images on receiving answers. Our results first show that user interface is the most common image content and undesired output is the most frequent purpose for sharing images. Moreover, these images essentially facilitate the understanding of 68% of sampled questions. Second, we find that discrepancy questions are more relatively frequent compared to those without images, but there are no significant differences observed in description length in all types of questions. Third, the quantitative results statistically validate that questions with images are more likely to receive accepted answers, but do not speed up the time to receive answers. Our work demonstrates the crucial role that images play by approaching the topic from a new angle and lays the foundation for future opportunities to use images to assist in tasks like generating questions and identifying question-relatedness.

==> comments.tex <==
\usepackage{datenumber}

\def\mybar#1{%%
  #1s & {\color{grey}\rule{#1cm}{8pt}}}

\newcommand\revdif[2]{\nb{#1}{\color{orange}#2}}
\newcommand\rev[2]{\nb{#1}{\color{red}#2}}
\newcommand{\nb}[2]{
	{
		{\color{red}{
				\fbox{\bfseries\sffamily\scriptsize#1}
				{\sffamily$\triangleright~${\it\sffamily #2}$~\triangleleft$}
	}}}
}


\definecolor{chestnut}{rgb}{0.8, 0.36, 0.36}


\newcommand\respond[2]{{\nb{#2}{\color{blue}#1}}}

\newcommand{\impacttext}[1]{{\color{red}#1}}
\newcommand{\rone}[1]{\colorbox{yellow}{\textbf{[#1]}}}
\newcommand\revise[1]{\nb{Revised}{\color{orange}#1}}
\newcommand\raula[1]{\nb{Raula}{\color{red}#1}}
\newcommand\ice[1]{\nb{Ice}{\color{magenta}#1}}
\newcommand\pick[1]{\nb{Pick}{\color{violet}#1}}
\newcommand\wang[1]{\nb{Wang}{\color{magenta}#1}}
\newcommand\yasu[1]{\nb{Yasu}{\color{orange}#1}}
\newcommand{\fixme}[1]{{\textcolor{red}{[FIXME] #1}}\xspace}
\newcommand{\cn}{{\color{violet}[citation required]}}
\newcommand{\tbd}{{\color{green}[To Be Done!]}}

\definecolor{chestnut}{rgb}{0.8, 0.36, 0.36}

%%% Date configs
% \newcounter{dateone}
% \newcounter{datetwo}

% \newcommand{\difftoday}[3]{%
%       \setmydatenumber{dateone}{\the\year}{\the\month}{\the\day}%
%       \setmydatenumber{datetwo}{#1}{#2}{#3}%
%       \addtocounter{datetwo}{-\thedateone}%
%       \the\numexpr-\thedatetwo/365\relax\space year(s),
%       \the\numexpr(-\thedatetwo - (-\thedatetwo/365)*365)/30\relax\space month(s)
% } 

\newcounter{dateone}\newcounter{datetwo}%
\newcommand{\daydifftoday}[3]{%
\setmydatenumber{dateone}{\the\year}{\the\month}{\the\day}%
\setmydatenumber{datetwo}{#1}{#2}{#3}%
\addtocounter{datetwo}{-\thedateone}%
\thedatetwo
}

